BMRetriever: Tuning Large Language Models as Better Biomedical Text Retrievers

Developing effective biomedical retrieval models is important for excelling at knowledge-intensive biomedical tasks but still challenging due to the deficiency of sufficient publicly annotated biomedical data and computational resources. We present BMRetriever, a series of dense retrievers for enhancing biomedical retrieval via unsupervised pre-training on large biomedical corpora, followed by instruction fine-tuning on a combination of labeled datasets and synthetic pairs. Experiments on 5 biomedical tasks across 11 datasets verify BMRetriever's efficacy on various biomedical applications. BMRetriever also exhibits strong parameter efficiency, with the 410M variant outperforming baselines up to 11.7 times larger, and the 2B variant matching the performance of models with over 5B parameters. The training data and model checkpoints are released at \url{https://huggingface.co/BMRetriever} to ensure transparency, reproducibility, and application to new domains.

==> section/syn-query-case-study.tex <==
\begin{table*}[t!]
\centering
\renewcommand\arraystretch{0.92}
\resizebox{\linewidth}{!}{
    \begin{tabular}{lp{16.5cm}}
       \toprule
       \multicolumn{2}{c}{\bf Synthetic Query Generation Example 1} \\
       \midrule
       \bf Provided Passage & AIMS: The aim of this study was to report the results of custom-made endoprostheses with extracortical plates plus or minus a short, intramedullary stem aimed at preserving the physis after resection of bone sarcomas in children.PATIENTS AND METHODS: Between 2007 and 2017, 18 children aged less than 16 years old who underwent resection of bone sarcomas, leaving ? 5 cm of bone from the physis, and reconstruction with a custom-made endoprosthesis were reviewed. Median follow-up was 67 months (interquartile range 45 to 91). The tumours were located in the femur in 11 patients, proximal humerus in six, and proximal tibia in one.RESULTS: The five-year overall survival rate was 78\%. No patient developed local recurrence. The five-year implant survival rate was 79\%. In all, 11 patients (61\%) developed a complication. Seven patients (39\%) required further surgery to treat the complications. Implant failures occurred in three patients (17\%) including one patient with aseptic loosening and two patients with implant or periprosthetic fracture. The preserved physis continued to grow at mean 3.3 cm (0 to 14). The mean Musculoskeletal Society score was 88\% (67\% to 97\%).CONCLUSION: Custom-made endoprostheses that aim to preserve the physis are a safe and effective option for preserving physeal growth, limb length, and joint function with an acceptable rate of complications. Cite this article: Bone Joint J 2019;101-B:1144-1150.\\
       \midrule
        \bf Generated Query & What is the survival rate of a physeal osteoprosthesis? \\
        \toprule
        \multicolumn{2}{c}{\bf Synthetic Query Generation Example 2} \\
        \midrule
        \bf Provided Passage & The aryl hydrocarbon receptor (AhR) is activated by the ligand, benzo[a]pyrene (B[a]P), a component of smoke that is implicated in lung carcinogenesis in humans. However, the role of B[a]P and AhR in lung cancer malignancy is not well known. In this study, we analyzed the effects of B[a]P and AhR in the 3D spheroids of human lung cancer cells in vitro. In these spheroids, B[a]P and AhR enhanced cancer cell proliferation. These results suggest that the AhR-dependent effects of B[a]P on cell proliferation may contribute to the adverse effects of continuous smoking with respect to lung cancer malignancy. \\
        \midrule
        \bf Generated Query & What compounds are involved in cell proliferation? \\
       \bottomrule
    \end{tabular}
%\end{center}
}
	\caption{Synthetic queries generated by GPT-3.5 based on the provided passages from PubMed.}
	\label{tab:syn_query_case_study}
\end{table*}

